KAPLAN: A 3D Point Descriptor for Shape Completion

We present a novel 3D shape completion method that operates directly on unstructured point clouds, thus avoiding resource-intensive data structures like voxel grids. To this end, we introduce KAPLAN, a 3D point descriptor that aggregates local shape information via a series of 2D convolutions. The key idea is to project the points in a local neighborhood onto multiple planes with different orientations. In each of those planes, point properties like normals or point-to-plane distances are aggregated into a 2D grid and abstracted into a feature representation with an efficient 2D convolutional encoder. Since all planes are encoded jointly, the resulting representation nevertheless can capture their correlations and retains knowledge about the underlying 3D shape, without expensive 3D convolutions. Experiments on public datasets show that KAPLAN achieves state-of-the-art performance for 3D shape completion.

==> tex/denoising.tex <==
\section{Point Cloud Denoising}
\label{sec:denoising}

% Show results how our local descriptor performs for point cloud denoising.
There two ways to think about the task of denoising here: 
\begin{itemize}
	\item either we say we start from a noisy point cloud and we want to correct only existing points. We do not introduce new clean/denoised points. We compute a \kaplan{} per point and we use only the final output depth predicition for the central pixel to denoise the point (for which \kaplan{} was computed). In that case, we don't introduce new points (density stay the same), we just correct position of the current existing points. We are then sure to keep scalability. 
	\item or we think about it in this way: we consider that we compute some noisy \kaplan{} (since it is \kaplan{} computed on noisy point cloud) and the network should extract features such it can recognize the non noisy structure behind that. Then it will predict clean points where needed. In that way, it is more an experiment that checks the representative power of our approach to generate non-noisy point cloud from noisy representation. In that case, we will introduce our own points (so we need to control the output density we want to have).So we need to ensure to introduce not too much points and that it doesn't explode. 
\end{itemize}


 
 

 


==> tex/discussion.tex <==


 
 
 

